LLM-Assisted Content Conditional Debiasing for Fair Text Embedding

Mitigating biases in machine learning models has become an increasing concern in Natural Language Processing (NLP), particularly in developing fair text embeddings, which are crucial yet challenging for real-world applications like search engines. In response, this paper proposes a novel method for learning fair text embeddings. First, we define a novel content-conditional equal distance (CCED) fairness for text embeddings, ensuring content-conditional independence between sensitive attributes and text embeddings. Building on CCED, we introduce a content-conditional debiasing (CCD) loss to ensure that embeddings of texts with different sensitive attributes but identical content maintain the same distance from the embedding of their corresponding neutral text. Additionally, we tackle the issue of insufficient training data by using Large Language Models (LLMs) with instructions to fairly augment texts into different sensitive groups. Our extensive evaluations show that our approach effectively enhances fairness while maintaining the utility of embeddings. Furthermore, our augmented dataset, combined with the CCED metric, serves as an new benchmark for evaluating fairness.

==> sec/intro_long.tex <==
\section{Introduction}
Embedding text into dense representations is a central
pursuit in modern Natural Language Processing (NLP) and Machine Learning. It has been widely applied in various applications such as sentiment analysis~\cite{dang2020sentiment}, recommendation systems~\cite{zhang2016collaborative}, search engines~\cite{palangi2016deep} and  modular use of
text embeddings for downstream tasks.
However, as language embedding becomes more ubiquitous in real-world applications, their latent biases may introduce biases in various subsequent tasks~\cite{packer2018text}. For instance, in web search engines~\cite{palangi2016deep,zerveas2022mitigating}, which rely on the similarity between query and text embeddings, embedding biases can persist in the retrieved results~\cite{baeza2018bias,biega2018equity,zerveas2022mitigating}. In legal information extraction~\cite{rabelo2022overview} and resume filtering~\cite{abdollahnejad2021deep}, the presence of biased text embeddings can potentially jeopardize the protection of marginalized groups' rights, including those related to gender, race, and other factors.
Unfortunately, various forms of biases, including gender, racial, and religious biases, have been identified in word/text embeddings generated by pre-trained language models (PLMs), as reported in several studies~\cite{bolukbasi2016man,nissim2020fair,liang2020towards,may2019measuring}. In the quest for optimal performance, practitioners frequently deploy PLMs without considering the potential consequences, leading to strong performance with the unseen cost of introducing bias into the process. Consequently, attaining fairness in text embedding models has become increasingly crucial.
 
Recent approaches to debiasing text embeddings~\cite{liang2020towards,kaneko2021debiasing} design post-training to mitigate biases before applying these embeddings in downstream tasks because training new sentence encoders each time a new bias is identified is inefficient. In addition, they focus on overcoming a major hurdle of achieving good “fairness and utility trade-off”~\cite{zhao2022inherent,deng2023fairness,zliobaite2015relation}. For instance,~\cite{liang2020towards,kaneko2021debiasing} decreases a word/sentence embedding’s projection on a linear bias subspace to achieve thus completely removing the semantic meanings from the text. ~\cite{yang2023adept} aims for a different approach by ensuring an equal distance from all embeddings to sensitive spaces. Nevertheless, these methods persist in pursuing independence between sensitive attributes and text embeddings, which do not effectively (find a sweet spot between ...) in this trade-off~\cite{zhao2022inherent}. 
%% add they completely removed the sensitive information.

% borrow the definition from paper Zhao and gordon, give a more clear definition, methods harm performance, not the fairness-utility it self


%%% leverage demographic labeled dataset can better design method to balance tradeoff cite related paper.
Recently, several studies~\cite{mary2019fairness,deng2023fairness,pogodin2022efficient} indicate that using datasets labeled with sensitive information to attain (what condition?  give a deeper illustration. we conditioned on content because we wish to maintain semantic information inside the text content, we cuts the pass conditional ) conditional independence offer a more effective balance in the tradeoff of representation learning. Yet, the scarcity of text datasets with sensitive labels~\cite{gallegos2023bias} limits the practical application of these findings. Although techniques like Counterfactual Data Augmentation (CDA)~\cite{zhao2018gender} attempt to annotate datasets by altering text samples to reflect diverse sensitive groups. For instance, this could involve modifying gendered words (\ie, swapping "She" with "He" and the reverse). This method may lead to the production of grammatically incorrect artificial instances~\cite{dinan2019queens}. (add contentthus harming the performance ) Recently, Large language models (LLMs) have been leveraged as training data generators for various NLP tasks~\cite{schick2021generating,shao2023synthetic}, however, they encounter the challenge of overcoming the inherent systematic biases present in LLMs~\cite{yu2023large}. 

In this paper, we propose a new method to balance the trade-off between fairness and model utility via \underline{C}ontent \underline{C}onditioned data \underline{G}eneration and sensitive attributes \underline{D}ebiasing (dubbed \ours{}). Specifically, in addressing bias in text embedding models while preserving their representational capabilities, \ours{} achieves conditional independence between sensitive attributes and text embeddings, conditioned on the text content. To combat data scarcity, this paper employs a rule-based, few-shot learning strategy to enable Large Language Models (LLMs) to generate fair data. This involves letting LLM conditioned on each given text, instructing to replace words associated with sensitive information in text samples by words from various sensitive groups performing similar roles (\ie, "girl" and "boy" for the male and female gender groups, respectively). We demonstrate the effectiveness of our method through extensive evaluations on several established debiasing benchmarks and downstream tasks. Our results reveal that our approach achieves a desirable trade-off, enhancing fairness without significantly compromising the representational capabilities of the embeddings. To our knowledge, this study is the first of its kind to employ LLMs in mitigating unfairness in text embedding models.


==> sec/method.tex <==
% \begin{table*}[t!]
% % \fontsize{10pt}{10pt}\selectfont
% \centering
% \caption{Evaluation results on debiasing performance. We test the debiased models on SEAT, CrowS-Pairs, and filtered StereoSet-Intrasentence, with the best result in bold.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccccc}
% \hline \hline \multirow{2}{*}{\begin{tabular}{l} 
% Datasets \\
% Method
% \end{tabular}} & \multicolumn{7}{c}{ SEAT $(0.00)$ the best } &\multicolumn{2}{c}{StereoSet} &\multicolumn{1}{c}{ CrowS-Pairs}\\
% \hline & $6$ & $6$-b & $7$ & $7$-b & $8$ & $8$-b & AVG & G-SS $(0.5)$  & A-SS$(0.5)$ &  SS $(0.5)$  \\
% \hline
% % \textbf{Baselines} & &  & &&  &  & & & & \\
% BERT & $0.37$ & $0.20$ & $0.42$ & $0.22$ & $-0.26$ & $0.71$ & $0.36$  & $59.66$& $58.24$& $55.73$\\
% DPCE & $-0.21$ &  $0.27$  &$0.44$ & $\textbf{0.07}$ & $0.25$ &$0.21$ &  $\underline{0.24}$& $56.72$& $52.96$ & $52.29$ \\
% ADEPT-F & $0.83$ & $-0.14$ & $0.63$ & $1.24$ & $0.43$ & $1.28$ & $0.76$ & $61.70$& $57.52$ & $51.91$ \\
% \hline
% % \textbf{Strategy Comparison} & &  & &&  & &  & & & \\
% \ours{}-CDA  & $\textbf{0.16}$ & $\textbf{0.03}$  & $0.43$ & $0.38$ & $0.47$  & $0.22$ & $0.29$ & $53.53$& $53.46$ & $46.95$\\
% % \ours{}-google  & $0.64$ & $-0.08$  & $0.51$ & $0.02$ & $0.13$  & $0.66$ & $0.34$ & $55.84$ & $54.16$ & \mathbf{50.38}$\\
% % \ours{}-google2  & $0.66$ & $-0.14$  & $0.20$ & $-0.23$ & $0.14$  & $0.03$ & $0.23$ & $56.20$ & $55.54$ & $51.53$\\
% \ours{}  & $0.35$ & $-0.11$  & $\textbf{-0.17}$ & $-0.15$ & $0.57$  & $0.06$ & $\textbf{0.23}$ &$53.60$ &$52.83$ & $47.71$\\
% % \hline
% % \ours{}  & $0.47$ & $-0.06$  & $-0.33$ & $0.55$ & $-0.17$  & $0.48$ & $0.34$  & $55.40$& $54.80$ & $\mathbf{49.62}$\\
% \hline\hline
% \end{tabular}
% }
% \label{tab:fairness}
% \end{table*}
\section{Method}
\subsection{Problem Setting}
This section outlines the problem of fairness in text embeddings. We define the key variables: $S$ represents the input text, $C$ the content\footnote{The texts 'he is a teacher' and 'she is a teacher' both inherently contain the same content $C$ = 'is a teacher'.}, and $f$ the text embedding model that produces the text embedding $C' = f(S)$. Sensitive attributes are denoted as $A =[a_1,..., a_{|A|}]$ (e.g., gender, race, age), words in the text related to attribute $a_i$ as $X^{a_i}$, and neutral words as $X^{n}$. A text is considered neutral ($S^{n}$) if it lacks sensitive words and is associated with attribute $a_i$ ($S^{a_i}$) based on its sensitive polarity~\cite{wang2023toward}. All notations are listed in Appendix Table~\ref{tab:Notation}.
\\
\textbf{Fairness Issue}: Fig.~\ref{fig:fair} (a) shows there exists an association between attributes $A$ and content variable $C$, if model $f$ superficially considers $A$ as a proxy for $C$, leading to issues of fairness.
\\
\textbf{Fairness Goal}: Mitigating fairness is not trivial, as we need to address not only bias mitigation but also the protection of the model's representation ability.  As shown in Fig.~\ref{fig:fair} (a), (1) our method aims to break the association between content $C$ and the sensitive attribute $A$. (2) we aim to preserve useful sensitive information in the text embedding. For example, in the case of a text about a father raising a child, its embedding should retain information about the father.
\subsection{Content Conditional Fairness Loss}
We propose to achieve conditional independence between sensitive attributes and content $A \perp C' ~|~ C$. The conditional independence allows prediction $C'$ to depend on $A$ but only through the content variable $C$, prohibiting abusing $A$ as a \textit{proxy} for $C$ thus mitigating the fairness issue while preserving the utility. 
Echoing the methodologies in previous research~\cite{hinton2002stochastic,yang2023adept}, we can define the probability $P(i|j)$ as the likelihood of variable $i$ selecting $j$ as its neighbor in the embedding space. Then conditional independence $A \perp C' ~|~ C$ can be represented as a content conditioned equal distance on the embedding space, as shown in Fig.~\ref{fig:fair} (b) and definition~\ref{def:fairness} (detailed proof in Appendix~\ref{sec:proof}) : 
% More specifically, rather than completely removing sensitive information, we allow text content $C$ to uniformly represent various sensitive attributes. Following~\cite{hinton2002stochastic,yang2023adept}, the probability $a_i$ conditioned on $C$ can be represent as $C$ would pick $a_i$ as its neighbor,
% we present a formal definition of fairness within the context of embedding spaces, detailed proof in Appendx~\ref{sec:proof}.
\begin{definition}(Content Conditional Equal Distance Fairness.)\label{def:fairness}
Let $S_C^n$ be a neutral text with the content $C$, assume $S_C^A = [S_C^{a_1}, S_C^{a_2},..., S_C^{a_{|A|}}]$ being a set of texts from all sensitive groups with the same content $C$. Then embedding model $f$ is content conditioned equal distance fair with respect to attribute $A$, for any $a_i,a_j \in A$:
    \begin{align}
        ||f(S_C^{a_i}) - f(S_C^{n})|| =  ||f(S_C^{a_j}) &- f(S_C^{n})||.
    \end{align}
    %%% give a motivation why the definition is true
    %%% find evidence that why equal distance is fair
\end{definition}
To align with this definition of fairness, we design a loss function $L_{bias}$ that aims to mitigate biases while preserving the representation ability of PLMs. For a sample pair $[S_C^{a_1},...,S_C^{a_{|A|}},S_C^{n}]$ :
\begin{align}\label{lossb}
\small
    L_{bias} = \sum_{i \in [A]} \sum_{j \not = i} & |dist(f(S_C^{a_i}),f(S_C^{n})) \nonumber   \\ &- dist(f(S_C^{a_j}),f(S_C^{n})) |,
\end{align}
where $dist(A,B) = \exp\left(- \frac{\lVert A - B \rVert^2}{2\rho^2} \right)$ measures the distance on the manifold~\cite{yang2023adept,hinton2002stochastic} (details in Appendix~\ref{sec:proof}), and $\rho$ is selected as the variance of the distance over the training dataset for normalization.  To further preserve the valuable information encoded in the model for downstream tasks, we design $L_{rep}$ to enforce similarity between the text embeddings processed by the fine-tuned model $f$ and those processed by the original model $f^{ori}$:
\begin{align}\label{lossr}
\small
    L_{rep} = ||f(S^{n}) - f^{ori}(S^n)||.
\end{align}
% give a visualization 
Thus, the overall training objective is:
\begin{align}\label{lossall}
\small
    L_{all} = L_{bias} + \beta * L_{rep}.
\end{align}
\subsection{Content Conditional Data Augmentation}\label{sec:ccd} 
\begin{algorithm}[t]
\caption{Data augmentation algorithm}\label{alg:aug}
\begin{algorithmic}
\Require text $S$, sensitive attributes $A$, sensitive word set $X^A$ in text, predefined sensitive word list $V$
\Ensure Augmented text $S^A$, neutral text $S^n$
\State \bf{Block I}: Augment Text into Different Sensitive Groups 
\State $S^A, S^n$ $\gets$ $h(X^A)$
\State $ = [[X_{a_m}^{a_i},...,X_{a_m}^{a_{j}}],[X_{n}^{a_i},...,X_{n}^{a_{j}}]]_{a_m \in A}$ 
\State \bf{Block II}: Rule Guided Prompt Searching
\For{$i$ in $1, \ldots, K$}
\State $g(S) \gets \arg\max_{a_i\in A} occ(S,V^{a_i})$
\If{$g(S^{a_i}) \not = i$}
\State Manually augmentation $S^{a_i}$
% \Else
% \State pass
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
To meet our goal in definition~\ref{def:fairness}, we augment a dataset into texts across various sensitive attributes $A$ linked to the same content variable $C$. The data augmentation algorithm is shown in Algorithm \ref{alg:aug}.
\\
\noindent\textbf{Augment Text into Different Sensitive Groups:}
% \bd{We facilitate text augmentation by using a pre-trained LLM to get sensitive and neutral texts. To avoid the LLM reproduce and augment biases wild, instead of generating texts, we replace sensitive words in texts with counterparts from different sensitive groups and neutral words. For a set of sensitive words $X^A = [X^{a_i}, \ldots, X^{a_j}]$, $a_i, a_j \in A$ in text $S$, the LLM $h$ replaces the set to sets of sensitive words from other sensitive groups and neutral words, which is shown as
% \begin{align}
%     h(X^A) = [[X_{a_m}^{a_i},...,X_{a_m}^{a_{j}}],[X_{n}^{a_i},...,X_{n}^{a_{j}}]]_{a_m \in A, n \not \in A},
% \end{align}
% where $a_m \in A$ represents other sensitive attributes, $n$ means a neutral attribute. Therefore, we can get all augmented sensitive texts $S^A$ and one augmented neutral text $S^n$ after word sets replacing. Examples are shown in Appendix Table~\ref{tab:generated}}
We facilitate text augmentation by using a pre-trained LLM to replace sensitive words with equivalents from different sensitive groups. 
\iffalse
Using LLMs to generate data may introduce biases, we instead empower the LLM to replace sensitive words with equivalents from different sensitive groups. 
\fi
As shown in Fig.~\ref{fig:fair} (a), for sensitive words $X^A = [X^{a_i},...,X^{a_j}], a_i, a_j \in A$ in text $S$, the LLM $h$ substitutes $X^A$ with words from different sensitive groups $h(X^A) = [[X_{a_m}^{a_i},...,X_{a_m}^{a_{j}}]]_{a_m \in A}$ respectively, creating augmented texts $S^A$ from all sensitive groups. We also generate a neutral version $S^{n}$ using neutral replacements, resulting in a dataset of texts from different groups $\mathcal{S}^{A}$ and a neutral text $S^{n}$. Examples are provided in Appendix Table~\ref{tab:generated}.
 \\
 \noindent\textbf{Rule Guided Prompt Searching:} 
Considering the impact of few-shot prompt tuning on LLM effectiveness, choosing the right prompts is essential for successful text augmentation. As shown in Fig.~\ref{fig:fair} (d), we first find inaccurately augmented texts whose augmented text's sensitive group mismatches its sensitive polarity~\cite{wang2023toward} computed by:
 \begin{align}\label{eq:p_check}
     g(S) = \arg\max_{a_i\in A} occ(S,V^{a_i}),
 \end{align}
where $occ$ counts occurrences of words from the sensitive words lists $V^{a_i}, a_i\in A$ in the sentence $S$, we assign polarity based on the most frequently mentioned group in $A$. A text $S^{a_i}$ is considered wrongly augmented if $g(S^{a_i}) \not = i$. We then manually augment such texts to create example prompts for better alignment and repeat the process. This process is iterated to select $K$ (ours 8) samples as few-shot prompts.
\\
\textbf{Data Augmentation Results:}
In this section, we show data samples augmented by our algorithm in Table~\ref{tab:generated}. Words associated with sensitive information in the text are replaced with corresponding words from all different sensitive groups and their neutral counterparts. Ultimately, we obtained a dataset with texts of content $C$ from all groups $A$ and neutral. 

\begin{table*}
\caption{We utilize LLM to augment text into three gender categories: Male, Female, and Neutral. Below are sample examples of the generated data, where words containing gender information are highlighted in colors: \textcolor{red}{red} for male, \textcolor{blue}{blue} for neutral, and \textcolor{orange}{orange} for female.}
\resizebox{\linewidth}{!}{%
 \begin{tabular}{c|c}
 \hline
 Gender & Generated Text \\
  \hline
 \multirow{4}{*}{Male} & 
But because \textcolor{red}{Rumsfeld} wanted to prove a point about transforming strategy.\\
& After championing the continuation of \textcolor{red}{his} hardline policy, \textcolor{red}{his} current strategy of negotiation is risky. \\
&  \textcolor{red}{He} has been very vocal in voicing discontent with the rule of Kirchner and that of \textcolor{red}{his husband} and predecessor, Néstor Kirchner.
\\
\hline
 \multirow{4}{*}{Neutral} & 
But because the \textcolor{blue}{individual} wanted to prove a point about transforming strategy. \\
& After championing the continuation of \textcolor{blue}{their} hardline policy, \textcolor{blue}{the} current strategy of negotiation is risky. \\
& \textcolor{blue}{They} have been very vocal in voicing discontent with the rule of Kirchner and that of \textcolor{blue}{their spouse} and predecessor, Néstor Kirchner. \\
\hline
 \multirow{4}{*}{Female} & 
But because \textcolor{orange}{Rachel} wanted to prove a point about transforming strategy. \\
& After championing the continuation of \textcolor{orange}{her} hardline policy, \textcolor{orange}{her} current strategy of negotiation is risky. \\
& \textcolor{orange}{She} has been very vocal in voicing discontent with the rule of Kirchner and that of \textcolor{orange}{her wife} and predecessor, Néstor Kirchner.  \\
\hline
\end{tabular} \\
}

\label{tab:generated}
\end{table*}


==> sec/problem.tex <==
\section{Problem Setting}
This section outlines the problem of fairness in text embeddings. We define notations: $S$ for input text, $C$ for the content, and $f$ for the text embedding model that generates content embedding $f(S)$. Sensitive attributes $A =[a_1,..., a_{|A|}]$ (e.g., gender, race, age) and $X^{a_i}$ for words related to attribute $a_i$, with $X^{n}$ as neutral words. A text is neutral ($S^{n}$) if it lacks sensitive words, and associated with attribute $a_i$ ($S^{a_i}$) based on its sensitive polarity. We list all notations in Appendix Table~\ref{tab:Notation} for reference.
\\
\textbf{Fairness Issue}: As shown in Fig.~\ref{fig:fair} (c), there exists a superficial association between attributes $\mathcal{A}$ and the content variable $C$, causing the model $f$ to superficially consider $A$ as a proxy for $C$, which leads to issues of fairness. 

